Embedding-based Silhouette Community Detection

Mining complex data in the form of networks is of increasing interest in many scientific disciplines. Network communities correspond to densely connected subnetworks, and often represent key functional parts of real-world systems. In this work, we propose Silhouette Community Detection (SCD), an approach for detecting communities, based on clustering of network node embeddings, i.e. real valued representations of nodes derived from their neighborhoods. We investigate the performance of the proposed SCD approach on 234 synthetic networks, as well as on a real-life social network. Even though SCD is not based on any form of modularity optimization, it performs comparably or better than state-of-the-art community detection algorithms, such as the InfoMap and Louvain algorithms. Further, we demonstrate how SCD's outputs can be used along with domain ontologies in semantic subgroup discovery, yielding human-understandable explanations of communities detected in a real-life protein interaction network. Being embedding-based, SCD is widely applicable and can be tested out-of-the-box as part of many existing network learning and exploration pipelines.

==> ex_proof.tex <==




\hl{Jan, a lahko predvsem od tu do konca sekcije pogledas ce zadeva drzi vodo? Poskusal sem zanalizirat kako se obnasa interval vrednosti z ozirom na upper bound (vsi k-ji)}
We next present a closed-form solution offering insight into potential speedups of the proposed optimization method with respect to na\"ive $k$ parameter sweep. Let $n$ be the total number of $k$ values considered. let $\alpha$ represent the interval, at which SCD considers $k$ values. For example, if $\alpha = 10$, every tenth $k$ shall be considered. Let $g(\alpha, n)$ denote the function representing the speedup of the SCD's optimization with respect to the na\"ive $k$ sweep. The $g$ can be expressed via the following equality:

\begin{align*}
  n &= g(\alpha, n) \cdot \big (\frac{n}{\alpha} + 2 \cdot (\alpha - 1) \big ) \\
  g(\alpha, n) &= \frac{n}{(\frac{n}{\alpha} + 2 \cdot (\alpha - 1))} = \frac{n \cdot \alpha}{n + 2 \cdot \alpha^{2} - 2 \cdot \alpha}  
\end{align*}

The obtained $g$ thus connects the total number of possible $k$ values ($n$), and the number of considered $k$ values (via $\alpha$).
The intuitiion behond the first equation is as follows.
The $(\frac{n}{\alpha} + 2 \cdot (\alpha - 1)$ part of the first equation represents the number of $k$ values checked by the proposed optimization. We are interested in a function ($g(\alpha,n)$), which connects the total number of possible steps $n$ with the number of steps conducted by SCD. Once expressed, $g(\alpha,n)$ offers the means to investigate the relation between $n$ and $\alpha$, indicating potentially relevant $\alpha$ estimations, given the starting $n$ (discussed next).
We next present a closed form solution connecting the $g$ (symbolic expression of speedup) with a constant speedup of $C$. We consider thus the following inequality:

\begin{align*}
  C < & g(\alpha, n)   = \frac{n \cdot \alpha}{n + 2 \cdot \alpha^{2} - 2 \cdot \alpha}\\
  n \cdot \alpha >& (n + 2 \cdot \alpha^{2} - 2 \cdot \alpha) \cdot C \\
  n \cdot  \alpha >& C \cdot n + C \cdot 2 \cdot \alpha^{2} - 2 \cdot C \cdot \alpha \\
  n >& \frac{C \cdot 2 \cdot \alpha (\alpha - 1)}{\alpha - C} = \frac{C \cdot 2 \cdot \alpha^{2} - C \cdot 2 \cdot \alpha}{\alpha - C}
\end{align*}

The closed form solution offers exact determination of speedup, offered by SCD over the na\"ive $k$ parameter sweep. We next discuss how the obtained inequality can be used to inspect when the SCD's optimization offers any speedup (at all). Such situation can be described by simply setting the $C = 1$. In this case,

\begin{equation*}
n > \frac{2 \cdot \alpha^{2} - 2 \cdot \alpha}{\alpha - 1} = 2 \cdot \alpha.
\end{equation*}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{opt2}
  \caption{Parameter space of $g(\alpha, n)$. The brighter the cell values, the larger the potential speedup.}
  \label{fig:opt}
\end{figure}

Thus, the proposed SCD's Silhouette optimization outperforms na\"ive sweep as soon as the number of considered $k$ values is larger than twice the selected $\alpha$ interval size. We further investigate a more general case accross a spectre of possible $n$ and $\alpha$ values. The cells in Figure~\ref{fig:opt} represent $g(\alpha,n)$ values---the speedup obtained given a pair of $n$ and $\alpha$. For the figure we considered $n$ valued between 1 and 10{,}000 and $\alpha$ valued between 1 and 1{,}000, as we believe such parameter range covers many real-world networks. It can be observed that up to 30x speedup can be obtained.

We finally estimate the value of $\alpha$ based on the input parameter $n$. This insight is based on the general expression for $g(\alpha,n)$, as stated in the previous paragraph. The $\alpha$ is estimated so that the value of $g$ is \emph{maximized}. As can be seen in Figure~\ref{fig:opt}, relatively small values of $\alpha$ (w.r.t values of $n$) yield the best performance. We next investigated, whether the closed form solution connecting the $\alpha$ and $n$ can be used to identify a suitable value of $\alpha$ based on $n$, the parameter of the approach. The rationale for this step is reduction of the number of hyperparameters, as to this point, both $\alpha$, as well as $n$ need to be specified by the user.

We derive the $\alpha$, used during actual SCD optimization as follows. First, we assume that the space of $\alpha$ values is real-valued. Even though in practice this is not the case, as the values of $k$ are natural numbers (positive), this assumption enables partial derivation with respect to $\alpha$, offering good approximation for the starting value when rounded to the nearest integer. Thus, we are interested in the solutions of the following equality:

\begin{equation*}
  0 = \frac{\partial g(\alpha,n)}{\partial \alpha}  =\frac{\partial (n \cdot \alpha)}{\partial \alpha ( n + 2 \cdot \alpha^{2} - 2 \cdot \alpha)}
\end{equation*}
%  0 &= n^{2} + 2 \cdot n \cdot \alpha^{2} - 2 \cdot \alpha \cdot n - 4 \cdot n \cdot \alpha^{2} + 2 \cdot n \cdot \alpha \\
%  - n^{2} &= - 2 \cdot n \cdot \alpha^{2}\\
%  \alpha &= \sqrt{\frac{n}{2}}
%\end{align}

After deriving and solving for $\alpha$, we obtain the folowing equality:

\begin{equation*}
\alpha = \sqrt{\frac{n}{2}}
\end{equation*}

In practice $n > 2$ (we are interested in finding at least two communities), thus the values of $\alpha$ are positive.
The obtained value for $\alpha$ thus represents an \emph{estimate} of the $k$ interval size, offering maximal speedup with respect to a given $n$. Note that in order to obtain this estimation, we assumed $\alpha$ is real-valued. The proposed SCD exploits this theoretical insight when parametrizing the interval of $k$ values, where the $\alpha$ is rounded to the nearest integer. Note that by using this estimation, SCD needs one parameter less. We next discuss the final step of the proposed methodology, where the obtained communities are \emph{interpreted} via semantic subgroup discovery.
